Faithful Simulation of Distributed Quantum Measurements with Applications in Distributed Rate-Distortion Theory

We consider the task of faithfully simulating a distributed quantum measurement, wherein we provide a protocol for the three parties, Alice, Bob and Eve, to simulate a repeated action of a distributed quantum measurement using a pair of non-product approximating measurements by Alice and Bob, followed by a stochastic mapping at Eve. The objective of the protocol is to utilize minimum resources, in terms of classical bits needed by Alice and Bob to communicate their measurement outcomes to Eve, and the common randomness shared among the three parties, while faithfully simulating independent repeated instances of the original measurement. To achieve this, we develop a mutual covering lemma and a technique for random binning of distributed quantum measurements, and, in turn, characterize a set of sufficient communication and common randomness rates required for asymptotic simulatability in terms of single-letter quantum information quantities. Furthermore, using these results we address a distributed quantum rate-distortion problem, where we characterize the achievable rate-distortion region through a single-letter inner bound. Finally, via a technique of single-letterization of multi-letter quantum information quantities, we provide an outer bound for the rate-distortion region.

==> Covering_Lemma.tex <==
\paragraph*{\textbf{Mutual Packing Lemma for POVMs}}
Another technique used to prove Theorem \ref{thm: dist POVM appx} is a quantum version of mutual packing lemma. In what follows, we describe the mutual packing lemma for quantum measurements. 
For a Hilbert Space $\mathcal{H}_{AB}$ consider a POVM of the form $M_A \tensor M_B$, where $(M_A, M_B)$ are two POVMs each acting on one  sub-system. The operators for $M_A$  and $M_B$
are denoted, respectively, by $\Lambda^A_u \in \mathcal{B(H_A)}, u\in \mathcal{U}$ and $\Lambda^B_v \in \mathcal{B(H_B)}, v\in \mathcal{V}$, where $\mathcal{U}$ and $\mathcal{V}$ are finite sets.  Fix a joint-distribution $P_{UV}$ on  the set of all outcomes $\mathcal{U} \times \mathcal{V}$. Fix rates $r_1, r_2>0$.  For each $l\in [1,2^{nr_1}]$, let $U^n(l)$ be a random sequence generated according to $\prod_{i=1}^n P_U$. Similarly, let $V^n(k)$ be a random sequence distributed according to $\prod_{i=1}^n P_V$, where $k\in [1,2^{nr_2}]$. Suppose  $U^n(l)$'s and  $V^n(k)$'s are independent. Define the following random operators:
\begin{equation*}
A_{u^n}\deq |\{l: U^n(l)=u^n\}|\Lambda^A_{u^n}, \quad B_{v^n}\deq |\{k : V^n(k)=v^n\}|\Lambda^B_{v^n} 
\end{equation*}
where $\Lambda^A_{u^n}=\bigotimes_i \Lambda^A_{u_i}$ and $\Lambda^B_{v^n}=\bigotimes_i \Lambda^B_{v_i}$.
\begin{lem}
%Suppose $M_A$ and $M_B$ are two POVMs acting on  $\mathcal{H}_{A}$ and  $\mathcal{H}_{B}$ with the set of outcomes $\mathcal{U}$ and $\mathcal{V}$, respectively. Given a density operator $\rho_{AB}$ in the Hilbert Space $\mathcal{H}_{AB}$, the measurement $M_A \tensor M_B$ produces a joint distribution $P_{UV}$ on  the set of all outcomes $\mathcal{U} \times \mathcal{V}$.  For each $l\in [1,2^{nr_1}]$ let $U^n(l)$ a random sequence generated according to $\prod_{i=1}^n P_U$. Similarly, let $V^n(k)$ be a random sequence distributed according to $\prod_{i=1}^n P_V$, where $k\in [1,2^{nr_2}]$. Suppose  $U^n(l)$'s and  $V^n(k)$'s are independent. 
For any $\epsilon>0$ and sufficiently large $n$, with high probability 
\begin{equation}
\| \sum_{(u^n, v^n)\in \mathcal{T}_\delta^{(n)}(U,V)} A_{u^n} \tensor B_{v^n}\|_\infty \leq \epsilon 
\end{equation}provided that $r_1+r_2< I(U;V)-\delta(\epsilon)$. 
\end{lem}
% \begin{proof}
% The proof is provded in \cite{ArXiv}.
% \end{proof}
\begin{proof}
From the triangle-inequality and the definition of $A_{u^n}$ and $B_{v^n}$, the norm in the lemma does not exceed the following
%
\begin{align*}
\sum_{l,k} \sum_{(u^n, v^n)\in \mathcal{T}_\delta^{(n)}(U,V)} & \hspace{-20pt} \11\{U^n(l)=u^n, V^n(k)=v^n\} \|\Lambda^A_{u^n} \tensor \Lambda^B_{v^n}\|_\infty\\
&\leq \sum_{l,k}\PP\{ (U^n(l), V^n(k))\in \mathcal{T}_\delta^{(n)}(U,V)\}
\end{align*}
where the last inequality holds since  $\Lambda^A_{u^n} \tensor \Lambda^B_{v^n} \leq I$. The proof completes from the classical mutual packing lemma. 
\end{proof}


% For such measurement define a canonical ensemble $\{\lambda_j, \hat{\rho}_j\}_{j\in [1,m]}$, where  
% \begin{align}
%     \lambda_j \deq \tr(\rho M_j)  \text{ and }  \hat{\rho}_j \deq \cfrac{1}{\lambda_j}\sqrt{\rho}M_j \sqrt{\rho}.
% \end{align}

% Let $\pi_{\rho}$ and $\pi_{w^n}$ denote the $\delta$-typical projector and conditional typical projectors defined for the ensemble $\{\lambda_j, \hat{\rho}_j\}$, where $w^n \in [1,m]^{\times n}$. For each $w \in [1,m]^{\times n}$, define 
% \begin{align*}
% \Lambda'_{w^n} = \pi_{\rho} \pi_{w^n} \hat{\rho}_{w^n} \pi_{w^n} \pi_{\rho}
% \end{align*}
% where $\hat{\rho}_{w^n} \deq \bigotimes \hat{\rho}_{w_i}$. Let $W^n$ be a sequence of IID random variables each distributed according to $\lambda_j$. Then $\EE[\hat{\rho}_{W^n}]=\rho^{\tensor n}$. Define $\sigma' \deq \EE[\Lambda'_{W^n}]$, where the expectation is taken with respect to $W^n$. Let $\hat{\pi}$ be the projector onto the subspace spanned by the eigen-states of $\sigma'$ that are larger than $\epsilon2^{-nS(\rho)}$. Define,
% \begin{align*}
% \Lambda_{w^n} \deq \Hat{\pi}\Lambda'_{w^n}\Hat{\pi} \text{ and } \sigma \deq \EE[\Lambda_{W^n}]
% \end{align*}
% Construct observables
% \begin{align*}
% A_{w^n} = 2^{-nR}\bigg((\sqrt{\rho_{\delta}})^{-1}\Lambda_{w^n}(\sqrt{\rho_{\delta}})^{-1}\bigg)
% \end{align*}

% Let $\mathcal{C}$ be a collection of  collection of sequences $w^n$. By $M_{\mathcal{C}}$ denote a collection of observables defined as $|\mathcal{C}|^{-1}A_{w^n}, w^n \in \mathcal{C}$.  

% \begin{lem}
% Suppose $\mathcal{C}$ is a collection of random vectors $W^n(l), l\in [1:2^{nR}]$ each distributed IID according to $\lambda_j, j\in [1,m]$. Then, $M_{\mathcal{C}}$ is a random sub-POVM such that for large enough $n$
% \begin{align*}
% \PP\Bigg\{ \tr\left(\sum_{w^n \in \mathcal{C}} 2^{-nR}A_{w^n} \rho^{\tensor n}\right)\geq 1-\epsilon \Bigg \} \geq 1-o(\epsilon)
% \end{align*}  
% holds if $R\geq  \mathcal{X}(\lambda_j, \hat{\rho}_j)+o(\epsilon)$.
% \end{lem}



==> POVM_Appx_Proof_OLD.tex <==
\subsection{Proof of the Theorem}

Consider a quantum system with the state described by the density operator $\rho_{AB}$ in the Hilbert Space $\mathcal{H}_{AB}$. Let $(M^{A}, M^B)$ be two POVMs as in the statement of the theorem.  

Let $\pi_{\rho_X}$ and $\pi^X_{u^n}$ denote the $\delta$-typical projector and conditional typical projectors defined for the canonical ensemble $\{\lambda^X_u, \hat{\rho}^X_u\}$, where $u^n \in \mathcal{U}^n$, \cite{winter}. Similarly, define $\pi_{\rho_Y}$ and $\pi^Y_{v^n}$ for the ensemble $\{\lambda^Y_v, \hat{\rho}^Y_v\}$. For each $u^n, v^n$, define 
\begin{align*}
\Lambda^{X'}_{u^n} = \uppi_{\rho_X} \pi^X_{u^n} \hat{\rho}^X_{u^n} \pi^X_{u^n} \pi_{\rho_X}\\
\Lambda^{Y'}_{v^n} = \pi_{\rho_Y} \pi^Y_{v^n} \hat{\rho}^Y_{v^n} \pi^Y_{v^n} \pi_{\rho_Y}
\end{align*}
where $\hat{\rho}^X_{u^n} \deq \bigotimes_{i} \hat{\rho}^X_{u_i}$ and $\hat{\rho}^Y_{v^n} \deq \bigotimes_{i} \hat{\rho}^Y_{v_i}$.  Let $(U^n,V^n)$ be a sequence of random variables, with uniform distribution over $\tau_{\delta}^{(n)}(U)$ and $\tau_{\delta}^{(n)}(V)$. Then $\EE[\hat{\rho}_{U^n}]=\rho_{X,\delta}^{\tensor n}$ and $\EE[\hat{\rho}_{V^n}]=\rho_{Y,\delta}^{\tensor n}$. Define $\sigma^{X'} \deq \EE[\Lambda^{X'}_{U^n}]$ and $\sigma^{Y'} \deq \EE[\Lambda^{Y'}_{V^n}]$, where the expectation is taken with respect to $U^n$ and $V^n$, respectively. Let $\hat{\pi}_X$ be the projector onto the subspace spanned by the eigen-states of $\sigma^{X'}$ that are larger than $\epsilon2^{-nS(\rho_X)}$. Similarly, define  $\hat{\pi}_Y$ for $\sigma^{Y'}$. Define,
\begin{align*}
\Lambda^X_{u^n} \deq \Hat{\pi}_X\Lambda^{X'}_{u^n}\Hat{\pi}_X \text{ and } \sigma_X \deq \EE[\Lambda^X_{U^n}]\\
\Lambda^Y_{v^n} \deq \Hat{\pi}_Y\Lambda^{Y'}_{v^n}\Hat{\pi}_Y \text{ and } \sigma_Y \deq \EE[\Lambda^Y_{V^n}]
\end{align*}
In what follows, we construct two random POVMs one for each encoder. Fix a positive integer $N$.  For each $\mu \in [1, N]$, randomly and uniformly select $2^{n\tilde{R}_1}$ and $2^{n\tilde{R}_2}$ sequences from the typical sets  $\tau_{\delta}^{(n)}(U)$ and $\tau_{\delta}^{(n)}(V)$, respectively. Let $U^{n,(\mu)}(l), V^{n,(\mu)}(k)$ represent the randomly selected sequences for each $\mu$, where $l\in [1, 2^{n\tilde{R}_1}]$ and $ k\in [1, 2^{n\tilde{R}_2}]$. Construct observables
\begin{align*}
A^{(\mu)}_{u^n} \delequal  \gamma^{(\mu)}_{u^n} \bigg(\sqrt{\rho_{X}}^{-1}\Lambda_{u^n}\sqrt{\rho_{X}}^{-1}\bigg)\quad  \text{ and  } \quad
B^{(\mu)}_{v^n} \delequal \zeta^{(\mu)}_{v^n} \bigg(\sqrt{\rho_{Y}}^{-1}\Lambda_{v^n}(\sqrt{\rho_{Y}}^{-1}\bigg)
\end{align*}
where 
\begin{align*}
 \gamma^{(\mu)}_{u^n}\deq  2^{-n\tilde{R}_1}|\{l: U^{n,(\mu)}(l)=u^n\}|\quad  \text{ and  } \quad
 \zeta^{(\mu)}_{v^n}\deq  2^{-n\tilde{R}_2}|\{k: V^{n,(\mu)}(k)=v^n\}| 
\end{align*}
 Then, for each $\mu \in [1,N]$ construct POVMs $M_B^{( n, \mu)}$ and $M_A^{( n, \mu)}$ as the following
\begin{align}
   M_A^{( n, \mu)}&= \{A^{(\mu)}_{u^n} : u^n \in \tau^n_\delta(U)\}, \quad  M_B^{(n, \mu)} = \{B^{(\mu)}_{v^n} : v^n \in \tau^n_\delta(V)\}.
\end{align} 

\subsection{Random Binning}
We introduce the quantum counterpart of the so-called \textit{binning} technique which has been widely used in the context of classical distributed source coding. Consider the POVMs $M_B^{( n, \mu)}$ and $M_A^{( n, \mu)}$. 
Fix binning rates $(R_1, R_2)$. Randomly partition the sets $\mathcal{U}^n$ and $\mathcal{V}^n$ into $2^{nR_1}$ and $2^{nR_2}$ equal size bins, respectively. For each $i\in [1,2^{nR_1}], j\in [1,2^{nR_2}]$, let $\mathcal{B}_1(i)$ and $\mathcal{B}_2(j)$ denote the $i^{th}$ and $j^{th}$ bins. Define the following POVMs 
\begin{align}
	    M_X^{( n, \mu)} \deq  \{\Gamma^{X,  (\mu)}_i: \Gamma^{X, ( \mu)}_i = \sum_{u^n \in \mathcal{B}_1(i)}A^{(\mu)}_{u^n},  i \in [1, 2^{nR_1}] \} \nonumber \\
	    M_Y^{( n, \mu)}\deq  \{\Gamma^{Y, ( \mu)}_j : \Gamma^{Y,( \mu)}_j = \sum_{v^n \in \mathcal{B}_2(j)}B^{( \mu)}_{v^n}, j \in [1, 2^{nR_2}] \}
\end{align}
Let $M_X^{(n)}=\frac{1}{N}\sum_\mu  M_X^{( n, \mu)}, M_Y^{(n)}=\frac{1}{N}\sum_\mu  M_Y^{( n, \mu)} $. We use $( M_X^{(n)},  M_Y^{(n)}) $ as the two POVMs for each encoder.  
\subsection{The mapping $\beta$ }
%Suppose the decoder used for the single-letter POVM $M_{XY}$ is a c-q channel represented by the mapping $\beta(u,v)\deq \tau_{u,v}$, where $u\in \mathcal{U}, v\in \mathcal{V}$ and $\tau_{u,v}$ is the reconstruction density operator for measurement outcomes $(u,v)$. 
We define a mapping $\beta$ acting on the outputs of $M_X^{(n)}\tensor M_Y^{(n)}$. For $\mu=1$, let us define $D_{i,j,\delta} \deq \{(l,k): (U^{n,(1)}(l),V^{n,(1)}(k)) \in A_{\epsilon}(P_{UV}) \text{ and } (U^{n,(1)}(l),V^{n,(1)}(k)) \in \mathcal{B}_1(i)\times \mathcal{B}_2(j)\}$ and $\alpha_{i,j} \deq |D_{i,j,\delta}|$. Define a function $F$ as  $F(i,j)=(U^{n,(1)}(l),V^{n,(1)}(k))$ if  $(k,l)$ is the only element of $D_{i,j,\delta}$; otherwise $F(i,j)=(u_0^n, v_0^n)$, where $(u_0^n, v_0^n)$ are arbitrary sequences. For each measurement outcome $(i,j)$, define the reconstructions state as $S_{i,j}\deq \tau_{F(i,j)} $. %Finally define $S_{(i,j)}\deq \frac{1}{N}\sum_{\mu}S^{(\mu)}_{i,j}$. 
%\begin{align}
%	    S_{ij} \deq \sum_{{(u^n,v^n) \in D_{i,j,\delta}}} \frac{1}{\alpha_{i,j}}\tau_{u^n v^n}.
%	\end{align}
The new decoder is a c-q channel given by $\tilde{\beta}^n(i,j)\deq S_{ij}$, where $i\in [0, 2^{nR_1}], j\in [0, 2^{nR_2}]$.

\subsection{Trace Distance}
We will show that $( M_X^{(n)},  M_Y^{(n)}) $ and $( M_X^{\tensor n},  M_Y^{\tensor n}) $ are close in trace distance. Let $A_{u^n} = \cfrac{1}{N}\sum_{\mu}A_{u^n}^{(\mu)}$ and $B_{v^n} = \cfrac{1}{N}\sum_{\mu}B_{v^n}^{(\mu)}$. More precisely, we will prove 

\begin{align}\label{eq:trace bound 1}
&\sum_{i, j} \sum_{ \substack{ u^n \in \mathcal{B}_1(i),\\ v^n\in \mathcal{B}_2(j)}}  \|\lambda_{u^n,v^n} \hat{\rho}^{\tensor n}_{u^n,v^n} \tensor \tau_{u^n, v^n} - (\sqrt{\rho}^{\tensor n} (A_{u^n} \tensor B_{v^n}) \sqrt{\rho}^{\tensor n}) \tensor S_{i,j}   \|_1\leq \epsilon
\end{align}
 From the triangle inequality, the term inside the above summation does not exceed
\begin{align*}
\|\lambda_{u^n,v^n} \hat{\rho}^{\tensor n}_{u^n,v^n} - (\sqrt{\rho}^{\tensor n} (A_{u^n} \tensor B_{v^n}) \sqrt{\rho}^{\tensor n}) \|_1+ \| (\sqrt{\rho}^{\tensor n} (A_{u^n} \tensor B_{v^n}) \sqrt{\rho}^{\tensor n}) \tensor(\tau_{u^n, v^n} -S_{i,j})\|_1.
\end{align*}
The second term above is further upper-bounded by 
\begin{align*}
&\frac{1}{N}\sum_{\mu} \| (\sqrt{\rho}^{\tensor n} (A^{(\mu)}_{u^n} \tensor B^{(\mu)}_{v^n}) \sqrt{\rho}^{\tensor n}) \tensor(\tau_{u^n, v^n} -S_{i,j})\|_1 \\
&= \frac{1}{N}\sum_{\mu} \| (\sqrt{\rho}^{\tensor n} (A^{(\mu)}_{u^n} \tensor B^{(\mu)}_{v^n}) \sqrt{\rho}^{\tensor n})\|_1 \times \|\tau_{u^n, v^n} -S_{i,j}\|_1 
\end{align*}
By definition, $\| (\sqrt{\rho}^{\tensor n} (A^{(\mu)}_{u^n} \tensor B^{(\mu)}_{v^n}) \sqrt{\rho}^{\tensor n})\|_1\leq \gamma^{(\mu)}_{u^n}\zeta^{(\mu)}_{v^n}$
% where 
% \begin{align*}
%  \gamma^{(\mu)}_{u^n}\deq  2^{-n\tilde{R}_1}|\{l: U^{n,(\mu)}(l)=u^n\}|\\
%  \zeta^{(\mu)}_{v^n}\deq  2^{-n\tilde{R}_2}|\{k: V^{n,(\mu)}(k)=v^n\}| 
% \end{align*}
Let $e(u^n,v^n)$ denote the bin numbers of $(u^n,v^n)$. Using the above argument, \eqref{eq:trace bound 1} is bounded by
\begin{align}\label{eq:trace bound 2}
&\sum_{u^n,v^n}  |\lambda_{u^n,v^n} \hat{\rho}^{\tensor n}_{u^n,v^n} - (\sqrt{\rho}^{\tensor n} (A_{u^n} \tensor B_{v^n}) \sqrt{\rho}^{\tensor n}) \|_1 + \frac{1}{N} \sum_{u^n,v^n}\sum_{\mu}\gamma^{(\mu)}_{u^n}\zeta^{(\mu)}_{v^n} \|\tau_{u^n, v^n} -S_{e(u^n,v^n)}\|_1    
\end{align}
Next, we derive an upper bound for the first summation in \eqref{eq:trace bound 2}. We use  Chernoff bound for  $\gamma^{(\mu)}_{u^n}\zeta^{(\mu)}_{v^n}$. If $N$ is as in the statement of the theorem, then with high probability,  the approximation   
\begin{align*}
\frac{1}{N}\sum_{\mu} \gamma^{(\mu)}_{u^n}\zeta^{(\mu)}_{v^n} \approx 2^{-n(H(U)+H(V)+o(\delta))},
\end{align*}
holds for any typical sequence $u^n$ and $v^n$. As a result, we can show that
\begin{align}\label{eq:bound for A B}
\| A_{u^n} \tensor B_{v^n} - 2^{-n(H(U)+H(V)+o(\delta))}\sqrt{\rho_X^{\tensor n} \tensor \rho_Y^{\tensor n}}^{-1} \Lambda_{u^n} \tensor \Lambda_{v^n}\sqrt{\rho_X^{\tensor n} \tensor \rho_Y^{\tensor n}}^{-1}\|_1\leq \epsilon'
\end{align}
We need the following lemma to proceed. 
\begin{lem} \label{lem:quantum jooint typicality}
Given typical sequences $u^n$ and $v^n$ the following inequalities hold
\begin{align*}
\| \rho^{\tensor n} (\rho_X^{\tensor n} \tensor \rho_Y^{\tensor n})^{-1} - 2^{-n I(\rho; \rho_X\tensor \rho_Y)+o(\delta)} \Pi_\delta\|_1 \leq \epsilon\\
\| \hat{\rho}_{u^n,v^n} - \hat{\rho}_{u^n} \tensor \hat{\rho}_{v^n}\|\leq \epsilon'
\end{align*}
where $I(\rho; \rho_X\tensor \rho_Y)\deq S(\rho_X)+S(\rho_Y)-S(\rho)$. 
\end{lem}
Note that for typical sequences $u^n$, $v^n$ we have $\lambda_{u^n} \approx 2^{-n(H(U)+o(\delta))}$ and $\lambda_{v^n} \approx 2^{-n(H(V)+o(\delta))}$. With this approximation, Lemma  \ref{lem:quantum jooint typicality} and \eqref{eq:bound for A B} each term in the first summation in \eqref{eq:trace bound 2} is bounded by
\begin{align}\nonumber
\|\lambda_{u^n,v^n} \hat{\rho}^{\tensor n}_{u^n,v^n} &- \lambda_{u^n}  \lambda_{v^n} 2^{-n (I(\rho; \rho_X\tensor \rho_Y)+o(\delta))}  \Pi_\delta \Lambda_{u^n} \tensor \Lambda_{v^n}\Pi_\delta \|_1\\\nonumber
&\leq \|\lambda_{u^n,v^n} \hat{\rho}^{\tensor n}_{u^n,v^n} - \lambda_{u^n}^X  \lambda_{v^n}^Y 2^{-n (I(\rho; \rho_X\tensor \rho_Y)+o(\delta))}  \Pi_\delta \hat{\rho}_{u^n}\tensor \hat{\rho}_{v^n}\Pi_\delta\|_1\\\label{eq:bound 3}
&+ \lambda_{u^n}  \lambda_{v^n} 2^{-n (I(\rho; \rho_X\tensor \rho_Y)+o(\delta))}  \|\Pi_\delta( \hat{\rho}_{u^n}\tensor \hat{\rho}_{v^n} -\Lambda_{u^n} \tensor \Lambda_{v^n})\Pi_\delta\|_1 
\end{align}
where the inequality holds by triangle inequality. The first term above equals 

\begin{align*}
    \|\lambda_{uv}\hat{\rho}_{uv} - \sqrt{\rho}A_u\otimes B_v \| & = \| \lambda_{uv}\hat{\rho}_{uv} - \sqrt{\rho}\big(A_u \otimes B_v + 2^{-n (H(U,V)} \sqrt{\rho_X \otimes \rho_Y}^{-1} (\Lambda_U \otimes \Lambda_V)\sqrt{\rho_X \otimes \rho_Y}^{-1}\big)\sqrt{\rho}\| \\
    & \leq \| \lambda_{uv}\hat{\rho}_{uv} - 2^{-n (H(U,V)}\sqrt{\rho}\sqrt{\rho_X \otimes \rho_Y}^{-1} (\Lambda_U \otimes \Lambda_V)\sqrt{\rho_X \otimes \rho_Y}^{-1}\sqrt{\rho}\big) \|_1 + \| \sqrt{\rho} \zeta \sqrt{\rho} \|_1  \\
    \end{align*}

\begin{align*}
\|\lambda_{u^n,v^n} \hat{\rho}^{\tensor n}_{u^n,v^n} & - 2^{-n I(\rho; \rho_X\tensor \rho_Y)+o(\delta)} \Pi_\delta \sqrt{\rho_X^{\tensor n}\tensor \rho_Y^{\tensor n}}^{-1} M_{u^n}^X\tensor M_{v^n}^Y  \sqrt{\rho_X^{\tensor n}\tensor \rho_Y^{\tensor n}}^{-1}\Pi_\delta \|_1 \\
&\leq  \epsilon'+\|\lambda_{u^n,v^n} \hat{\rho}^{\tensor n}_{u^n,v^n} -  \Pi_\delta\sqrt{\rho^{\tensor n}}^{-1}M_{u^n}^X\tensor M_{v^n}^Y  \sqrt{\rho^{\tensor n}}^{-1} \Pi_\delta \|_1\\
& =\epsilon'+\|\lambda_{u^n,v^n} \hat{\rho}^{\tensor n}_{u^n,v^n} - \lambda_{u^n,v^n} \Pi_\delta \hat{\rho}^{\tensor n}_{u^n,v^n} \Pi_\delta \|_1\\
&\leq \epsilon'+\lambda_{u^n,v^n} \delta
\end{align*}
For the first inequality we replaced $\rho_X^{\tensor n}\tensor \rho_Y^{\tensor n}$ with $\rho^{\tensor n}$ and applied Lemma \ref{lem:quantum jooint typicality}. The second term in \eqref{eq:bound 3} is bounded by
\begin{align*}
\lambda_{u^n}  \lambda_{v^n} \|\Pi_\delta( \hat{\rho}_{u^n}\tensor \hat{\rho}_{v^n} -\Lambda_{u^n} \tensor \Lambda_{v^n})\Pi_\delta\|_1  &\leq \lambda_{u^n}  \lambda_{v^n} \|\hat{\rho}_{u^n}\tensor \hat{\rho}_{v^n} -\Lambda_{u^n} \tensor \Lambda_{v^n}\|_1  \\
&= \lambda_{u^n}  \lambda_{v^n} \|\hat{\rho}_{u^n}-\Lambda_{u^n} \|_1 \times \|\hat{\rho}_{v^n}-\Lambda_{v^n} \|_1 
\end{align*}
As a result \eqref{eq:trace bound 2} is bounded by 
\begin{align*}
&\sum_{i, j} \sum_{ \substack{ u^n \in \mathcal{B}_1(i),\\ v^n\in \mathcal{B}_2(j)}} \lambda_{u^n}  \lambda_{v^n} \|\hat{\rho}_{u^n}-\Lambda_{u^n} \|_1 \times \|\hat{\rho}_{v^n}-\Lambda_{v^n} \|_1+ \frac{1}{N} \sum_{u^n,v^n}\sum_{\mu}\gamma^{(\mu)}_{u^n}\zeta^{(\mu)}_{v^n} \|\tau_{u^n, v^n} -S_{e(u^n,v^n)}\|_1  +o(\epsilon'+\delta)\\
&=\left( \sum_{u^n \in \tau_\delta(U)}  \lambda_{u^n}  \|\hat{\rho}_{u^n}-\Lambda_{u^n} \|_1\right) \times \left(\sum_{v^n \in \tau_\delta(V)}  \lambda_{v^n}  \|\hat{\rho}_{v^n}-\Lambda_{v^n} \|_1\right)\\&\quad + \frac{1}{N} \sum_{u^n,v^n}\sum_{\mu}\gamma^{(\mu)}_{u^n}\zeta^{(\mu)}_{v^n} \|\tau_{u^n, v^n} -S_{e(u^n,v^n)}\|_1  +o(\epsilon'+\delta)
\end{align*}
Next, we use Theorem (\ref{extrinsic}) to bound the first two term above. For that we set $\tilde{R}_1 \geq I(X; R)_{\sigma}$ and $\tilde{R}_2 \geq I(Y;R)_{\sigma}$. As a result of Theorem (\ref{extrinsic}), the first two terms are sufficiently small. Hence, it remains to bound the last summation above. For that we have 
\begin{align*}
&\frac{1}{N} \sum_{u^n\in \tau_\delta^n(U),v^n\in \tau_\delta^n(U)}\sum_{\mu}\gamma^{(\mu)}_{u^n}\zeta^{(\mu)}_{v^n} \|\tau_{u^n, v^n} -S_{e(u^n,v^n)}\|_1 
\end{align*}
Suppose $e(u^n,v^n)=(I,J)$. According to the construction of the proposed decoder, the trace norm inside the summation is upper bounded by the following indicator function:
\begin{align*}
\11\bigg\{\exists (\tilde{l}, \tilde{k})\in D_{I,J, \delta}: (U^{n, (1)}(\tilde{l}),V^{n, (1)}(\tilde{k}))\in \tau_\delta^n(UV), U^{n, (1)}(\tilde{l})\neq u^{n}, V^{n, (1)}(\tilde{k})\neq v^{n}  \bigg\}
\end{align*}
Denote such indicator function by $\11_{(I,J)}$. Note that this indicator function can be viewed as a random variable which is independent of $\gamma^{(\mu)}_{u^n}\zeta^{(\mu)}_{v^n}$ for $\mu >1$. This is due to the fact the binning is done independent of the random codewords and that the random variables $(U^{n,(\mu)}(l), V^{n,(\mu)})$ are independent for different $\mu$'s. As a result the above summation is bounded by  
\begin{align*}
&\frac{1}{N}+\frac{1}{N} \sum_{u^n\in \tau_\delta^n(U),v^n\in \tau_\delta^n(V)}\sum_{\mu>1} \gamma^{(\mu)}_{u^n}\zeta^{(\mu)}_{v^n} \11_{e(u^n, v^n)}
\end{align*}
By Chernoff bound the above summation is bounded by 
\begin{align*}
&\frac{1}{N}+\frac{N-1}{N}(1-\epsilon) \sum_{u^n\in \tau_\delta^n(U),v^n\in \tau_\delta^n(V)}\frac{1}{\| \tau_\delta^n(U)\|}\frac{1}{\| \tau_\delta^n(V)\|} \11_{e(u^n, v^n)}\\
&=\frac{1}{N}+\frac{N-1}{N}(1-\epsilon) \sum_{i,j} \big(\sum_{u^n\in \mathcal{B}_1(i),v^n\in \mathcal{B}_2(j)} \frac{1}{\| \tau_\delta^n(U)\|}\frac{1}{\| \tau_\delta^n(V)\|}\big) \11_{i,j}\\
&=\frac{1}{N}+\frac{N-1}{N}(1-\epsilon) \sum_{i,j} 2^{-n(r_1+r_2)} \11_{i,j}\\
%&\leq \frac{1}{N}+\frac{N-1}{N}(1-\epsilon)\PP(\11\bigg\{\exists (\tilde{l}, \tilde{k})\in D_{I,J, \delta}: (U^{n, (1)}(\tilde{l}),V^{n, (1)}(\tilde{k}))\in \tau_\delta^n(UV), U^{n, (1)}(\tilde{l})\neq u^{n}, V^{n, (1)}(\tilde{k})\neq v^{n}  \bigg\})
\end{align*}
Applying the Chernoff bound for IID random variables $\11_{(i,j)}$ gives the following upper bound
\begin{align*}
&\frac{1}{N}+\frac{N-1}{N}(1-\epsilon)^2 \EE[ \11_{1,1}]\leq\\
& \frac{1}{N}+\dfrac{N-1}{N}(1-\epsilon)^2 \PP\bigg\{\exists (\tilde{l}, \tilde{k}): (U^{n, (1)}(\tilde{l}),V^{n, (1)}(\tilde{k}))\in \tau_\delta^n(UV), U^{n, (1)}(\tilde{l})\in \mathcal{B}_1(1), U^{n, (1)}(\tilde{k})\in \mathcal{B}_2(1)  \bigg\}
\end{align*}
Since $U^n$ and $V^n$ are generated independently, we can apply the mutual packing lemma \cite{elGamal}. As a result the above probability approaches zero as $n\rightarrow \infty$ if $r_1+r_2 \leq I(U;V)$. 

To sum-up, we showed that the trace distance \eqref{eq:trace bound 1} is sufficiently small if the following bounds hold:
\begin{align*}
\tilde{R}_1&\geq I(X; R)_{\sigma}\\
\tilde{R}_2&\geq I(Y; R)_{\sigma}\\
(\tilde{R}_1-R_1)+(\tilde{R}_2-R_2) &\leq I(U;V)_{\sigma}
\end{align*}
These bounds imply the same bound as in the statement of the theorem. Hence, the proof is complete. 

==> Proof_Covering_lem.tex <==
\begin{proof}
By definition, the summation in the above equals to $\sum_{w^n \in \mathcal{C}} 2^{-nR}\tr\{\Lambda_{w^n}\}$. We find a constant $d>0$, and then use Chernoff operator bound on a $d \Lambda_{w^n}$. For that, we first find $d>0$ such that $\Lambda_{w^n} \leq \dfrac{1}{d}\hat{\pi}$. 

Let $\pi_{\hat{\rho}_j}^l$ be the typical projector of $\hat{\rho}_j$. Then, $\pi_{\hat{\rho}_j}^l \hat{\rho}_i^{\tensor l}\pi_{\hat{\rho}_j}^l \leq \frac{1}{d_j}\pi_{\hat{\rho}_j}^l$, where $d_j \geq  2^{l(S(\hat{\rho}_j )- \epsilon)}$.
For any vector $w^n$, let $N(j|w^n)$ denote the size of the set $\{i\in [1,n]: w_i=j\}$, where $j\in [1,m]$. Also, let $t(j|w^n)\deq \frac{1}{n}N(j|w^n)$. Therefore, we have	 
\begin{align}
     \pi_{w^n} \hat{\rho}_{w^n} \pi_{w^n} &= \Motimes_j \pi_{\hat{\rho}_j}^{N(j|w^n)}{\hat{\rho}}_j^{\Motimes N(j|w^n)}\pi_{\hat{\rho}_j}^{N(j|w^n)} \nonumber \\
    & \leq \Motimes_{j}  \cfrac{1}{d_j} \pi_{\hat{\rho}_j}^{N(j|w^n)} \nonumber \\
    & = \cfrac{1}{d_1d_2 ... d_m } \pi_{w^n}
\end{align}
where $d_j \geq 2^{nt(j|w^n)(S(\hat{\rho}_j )- \epsilon)}$. If $ w^n \in\tau_{\delta}(\lambda)$, then $|t(j|w^n)-\lambda_j|\leq \frac{\delta}{m}$. As a result, $d_j \geq 2^{n\lambda(S(\hat{\rho}_j )- \epsilon')}$, where $\epsilon'=\epsilon+\frac{\delta}{m} S(\hat{\rho}_j )$. This implies that for typical sequence $w^n$
\begin{align}
 \pi_{w^n} \hat{\rho}_{w^n} \pi_{w^n}  \leq  \frac{1}{d}  \pi_{w^n}
\end{align}
where $ d=2^{n (\sum_j \lambda_j S(\hat{\rho_j})+ o(\delta))}$. Therefore, $\Lambda_{w^n} \leq \frac{1}{d}\Hat{\pi} \pi_{w^n} \Hat{\pi} \leq \frac{1}{d}\Hat{\pi}$.
Next, we apply Chernoff operator bound on the operators $d\Lambda_{w^n}, w^n \in \mathcal{C} $. Such operators satisfy the necessary conditions for  Chernoff operator bound. For that,  
\begin{align}
    & 0 \leq d \Lambda_{w^n} \leq \Hat{\pi}, \qquad  \mathbb{E}[d \Lambda_{w^n}] = d \sigma \geq \cfrac{d\epsilon}{D}\Hat{\pi}
\end{align}
where $ D \geq 2^{nS(\rho) + \epsilon''}$. Further, from Chernoff Bound we know, 
% \begin{align}
%     \cfrac{1}{2^{nR}} \sum_{w^n \in \mathbb{C}} \Lambda_{w^n} \approx \mathbb{E}[\Lambda_{w^n}] = \sigma \text{ with high probability}.
% \end{align} And
\begin{align}
    \PP\Bigg\{\cfrac{1}{2^{nR}}\sum_{i=1}^{2^{nR}} \Lambda_{w^n(i)} \in [(1-\epsilon)\sigma , (1+\epsilon)\sigma] \Bigg\} & = \PP\Bigg\{\cfrac{1}{2^{nR}}\sum_{i=1}^{2^{nR}}d \Lambda_{w^n(i)} \in [(1-\epsilon)d\sigma , (1
    +\epsilon)d\sigma] \Bigg\}\nonumber \\
    & \geq 1- 2 \tr( \hat{\pi}) \Bigg{(}  \exp{\cfrac{-2^{nR}\epsilon^2\dfrac{\epsilon d}{D}}{4 \ln{2}}} \Bigg{)} \nonumber \\
 %   & \geq 1- 2D \exp{\cfrac{-2^{nR}\epsilon^2\dfrac{\epsilon d}{D}}{4 \ln{2}}} \Bigg{)} \nonumber \\
    & \geq 1- 2\cdot 2^{nS(\rho)} 
    \exp{- \cfrac{\epsilon^3}{4 \ln{2}} 2^{n[R-\chi(\lambda_j,\hat{\rho}_j)]}} \nonumber
\end{align}

Therefore, if $ R \geq \chi(\lambda_j,\hat{\rho}_j) + \epsilon'' $, then for large enough $n$ and  with high probability 
\begin{align}\label{eq:trace lambda}
\cfrac{1}{2^{nR}}\sum_{i=1}^{2^{nR}} \tr( \Lambda_{w^n(i)}) \geq (1-\epsilon)\tr(\sigma) 
\end{align}
In what follows, we show that $\tr(\sigma) \approx 1$. Note that $\tr(\sigma)=\tr(\hat{\pi}\sigma')=\tr(\sigma')-\tr((I-\hat{\pi})\sigma')$. Note that Schmidt rank of $\sigma'$ is at most $\tr(\phi_p)\leq 2^{n (S(\rho)+\delta)}$. Therefore,$\tr((I-\hat{\pi})\sigma') \leq \frac{\epsilon}{D} 2^{n (S(\rho)+\delta)} \leq \epsilon$. This implies that $\tr(\sigma) \geq  \tr(\sigma') -\epsilon$. Note that $\sigma'=\EE[\tr(\Lambda'_{W^n})]$.  Applying Corollary 9.1.1 \cite{book_quantum} yields    
\begin{align*}
\tr( \sigma')&= \tr(\pi_{\rho}  \EE[\pi_{w^n} \hat{\rho}_{w^n} \pi_{w^n}])\\
&\geq \tr(\pi_{\rho} \rho) -\frac{1}{2} \|\EE[\pi_{w^n} \hat{\rho}_{w^n} \pi_{w^n}] - \rho\|_1\\
&= \tr(\pi_{\rho} \rho) - \frac{1}{2} \|\EE[\pi_{w^n} \hat{\rho}_{w^n} \pi_{w^n} - \hat{\rho}_{w^n}]\|_1
\end{align*} 
 From triangle inequality, the last term in the above inequality does not exceed the following 
 \begin{align*}
 \EE[\|\pi_{w^n} \hat{\rho}_{w^n} \pi_{w^n} - \hat{\rho}_{w^n}\|_1].
 \end{align*}
Note that $\EE[\tr(\pi_{w^n} \hat{\rho}_{w^n})]\geq 1-\delta$. Hence, using the gentle lemma 9.4.3 in \cite{book_quantum},  the above quantity is upper bounded by $2\sqrt{\delta}$. Hence, $\tr( \sigma')\geq \tr(\pi_{\rho} \rho)- 2\sqrt{\delta} \geq 1-\delta-2\sqrt{\delta}$.  Finally, using the above argument, the right-hand side of  \eqref{eq:trace lambda} is larger than $(1-\epsilon)( 1-\delta-2\sqrt{\delta}-\epsilon)$.  This completes the proof. 

\end{proof}

==> binning.tex <==
%% Binning Technique 
\subsection{Proof Techniques}\label{sec:proofTechnqs}
\paragraph*{\textbf{Binning for POVMs}}
We introduce a quantum-counterpart of the classical binning technique used to prove Theorem \ref{thm: dist POVM appx}.
Here, we describe this technique. 

Consider a POVM $M$ with observables $\{ \Lambda_{\alpha_1},\Lambda_{\alpha_2}, .. , \Lambda_{\alpha_N} \}$.  Given $K$ for which $N$ is divisible, partition $[1,N]$ into $K$ equal bins and for each $i \in [1,K] $ , let $B(i)$ denote the $i^{th}$ bin. The binned POVM $\tilde{M}$ is given by the collection of operators $\{\tilde{\Lambda}_{\beta_1}, \tilde{\Lambda}_{\beta_2}, .. , \tilde{\Lambda}_{\beta_{K}} \}$ where $\tilde{\Lambda}_{\beta_i}$ is defined as 
\begin{equation}
    \tilde{\Lambda}_{\beta_i} = \sum_{ j \in \mathcal{B}(i)} \Lambda_{\alpha_j}. \nonumber
\end{equation}
Using the fact that $\Lambda_{\alpha_i}$ are self-adjoint and positive $\forall i\in [1,N]$ and $\sum_{i=1}^N \Lambda_{\alpha_i} = I$, (which is because $M$ is a POVM); it follows that $\tilde{M}$ is a valid POVM.

==> oldProofs.tex <==
\subsection{Proof of Lemma \ref{lem:nf_SoftCovering}} \label{lem:nf_SoftCovering_Proof}
\begin{proof}
Consider the trace norm expression given in \eqref{eq:nf_SoftCovering_Term}. This expression can be upper bounded using triangle inequality as 
\begin{align}
         &\left\|\sum_{w^n}\lambda_{w^n}\mathcal{T}_{w^n} - \cfrac{1}{2^{n(R+C)}}\cfrac{(1-\varepsilon)}{(1+\eta)}\sum_{l,\mu} \mathcal{T}_{W^n(l,\mu)}\right\|_1 \nonumber \\
         & \hspace{20pt} \leq \left \|\sum_{w^n}\lambda_{w^n}\hat{\rho}_{w^n}  \tensor \sigma_{w^n} - \cfrac{(1-\varepsilon)}{(1+\eta)}\sum_{w^n\in \TDeltaN(W)}\tilde{P}_{W^n}(w^n)\hat{\rho}_{w^n}  \tensor \sigma_{w^n}\right \|_1 \nonumber \\ 
    & \hspace{40pt}+  \left\|\cfrac{(1-\varepsilon)}{(1+\eta)} \left(\sum_{w^n\in \TDeltaN(W)}\tilde{P}_{W^n}(w^n)\hat{\rho}_{w^n}  \tensor \sigma_{w^n} - \cfrac{1}{2^{n(R+C)}}\sum_{l,\mu} \hat{\rho}_{W^n(l,\mu)}\tensor\sigma_{W^n(l,\mu)}\right)\right \|_1 \label{eq:nf_SoftCovering_TermSplit}
    \end{align}
    
\noindent Consider the following bounds on the first term in  (\ref{eq:nf_SoftCovering_TermSplit}). 
\begin{align}
     \left \|\sum_{w^n}\lambda_{w^n}\hat{\rho}_{w^n}  \tensor \sigma_{w^n} \right . & \left . - \cfrac{(1-\varepsilon)}{(1+\eta)}\sum_{w^n\in \TDeltaN(W)}\tilde{P}_{W^n}(w^n)\hat{\rho}_{w^n}  \tensor
    \sigma_{w^n}\right \|_1 \nonumber \\
    & \leq \left \|\sum_{w^n\in \TDeltaN(W)}\lambda_{w^n}\left(1-\cfrac{1}{(1+\eta)}\right)\hat{\rho}_{w^n}  \tensor \sigma_{w^n} \right \|_1 + \left \| \sum_{w^n \notin \TDeltaN(W)}\lambda_{w^n}\hat{\rho}_{w^n}  \tensor \sigma_{w^n}\right \|_1 \nonumber\\
    & \leq \left(\cfrac{\eta}{1+\eta}\right)\sum_{w^n\in \TDeltaN(W)}\lambda_{w^n}\underbrace{\left \|\hat{\rho}_{w^n}  \tensor \sigma_{w^n}\right \|_1}_{=1} + \sum_{w^n \notin \TDeltaN(W)}{\lambda_{w^n}}\underbrace{\left \|\hat{\rho}_{w^n}  \tensor \sigma_{w^n}\right \|}_{=1}\nonumber \\ 
    & \leq \left(\cfrac{\eta}{1+\eta}\right) + {\varepsilon} \leq \eta + \varepsilon = \varepsilon_1 \label{eq:ensemble2}
\end{align}
where $ \varepsilon_1 \searrow 0 $ as $ \epsilon \searrow 0 $.
%Using the upper bound from (\ref{eq:ensemble2}) in (\ref{eq:ensemble}), we get
%\begin{align}
%&\left \|\sum_{x^n,w^n}  \left[\lambda_{w^n}\hat{\rho}_{w^n} P^n_{X|W}(x^n|w^n) \tensor \ketbra{x^n} - \frac{1}{2^{nC}}\sum_{\mu =1}^{M}\gamma^{(\mu)}_{w^n}\hat{\rho}_{w^n}P^n_{X|W}(x^n|w^n) \tensor \ketbra{x^n} \right]\right \|_{1} \nonumber \\ 
%& \leq \varepsilon_1 +  \left \|\sum_{w^n \in \TDeltaN(W)}\tilde{P}_{W^n}(w^n)\hat{\rho}_{w^n}  \tensor \sigma_{w^n} - \cfrac{1}{2^{n(R+C)}}\sum_{l,\mu} \hat{\rho}_{W^n(l,\mu)}\tensor\sigma_{W^n(l,\mu)}\right \|_1 \label{eq:softCoveringTerm}
%\end{align}

\noindent Now consider the second term in (\ref{eq:nf_SoftCovering_TermSplit}). Using covering lemma from \cite{Wilde_book}, this can be bounded as follows.
Consider the ensemble given by $\{\tilde{P}_{W^n}({w^n}),\mathcal{T}_{w^n}\}$, where $ \tilde{P}_{W^n}({w^n}) $ follow from the definition in (\ref{eq:P_w^n}) and $  \mathcal{T}_{w^n} = \bigtensor_{n}\mathcal{T}_{w}  $ where $  
    \mathcal{T}_{w} = \hat{\rho}_{w}  \tensor \sigma_{w}. $
Furthermore, for all $w^n \in \TDeltaN(W)$, let $\Pi$ and $\Pi_{w^n}$ denote the projectors onto the typical subspace of $\mathcal{T}$ and $\mathcal{T}_{w^n}$, respectively, where $ \mathcal{T} = \sum_{w^n}\lambda_{w^n}\mathcal{T}_{w^n}. $
From the definition of typical projectors, for any $ \epsilon_1 \in (0,1) $ we have for sufficiently large $ n $, the following inequalities satisfied:
\begin{align}
    \Tr{\Pi\mathcal{T}_{w^n}} &\geq 1-\epsilon_1, \nonumber \\
    \Tr{\Pi_{w^n}\mathcal{T}_{w^n}} &\geq 1-\epsilon_1, \nonumber \\
    \Tr{\Pi} &\leq D \nonumber \\
    \Pi_{w^n}\mathcal{T}_{w^n}\Pi_{w^n} & \leq \frac{1}{d}\Pi_{w^n} \label{eq:coveringHyp}
\end{align}
where $D = 2^{n(S(\mathcal{T})+\delta_1)}$ and $ \displaystyle d = 2^{n\left[\left(\sum_{w}\lambda_w S(\mathcal{T}_{w})\right)+\delta_2\right]}$, and $ \delta_1 \searrow 0, \delta_2 \searrow 0 $ as $ \epsilon_{1} \searrow 0 $.
From the statement of the covering lemma, we know that for an ensemble $\{\tilde{P}_{W^n}(w^n), \mathcal{T}_{w^n}\}_{w^n \in \mathcal{W}^n}$, if there exists projectors $\Pi$ and $\Pi_{w^n}$ such that they satisfy the set of inequalities in (\ref{eq:coveringHyp}), then for any $\epsilon_2 > 0$,  sufficiently large $n$ and $n(R+C) > \log_2{\frac{D}{d}}$, the obfuscation error, defined as 
\begin{align}
    \left \|\sum_{w^n}\tilde{P}^n_W(w^n)\mathcal{T}_{w^n} - \cfrac{1}{2^{R+C}}\sum_{l,\mu}\mathcal{T}_{W^n(l,\mu)}\right \|_1
\end{align}
can be made smaller than $\varepsilon_2$ with high probability. 
This gives us the the following rate constraints $R + C \geq S({\sum_{w}\lambda_w\mathcal{T}_{w}}) - \sum_{w}\lambda_{w} S(\mathcal{T}_{w}) + \delta' = \chi\left(\{\lambda_w\},\{\hat{\rho}_{w}\tensor\sigma_{w}\}\right) + \delta' = I(RX;W)_{\sigma} + \delta'$.
\end{proof}

